Uniform difference between the length spectra of Out(F2) and the genus two handlebody group

In this paper, we analyze the natural homomorphism from the genus g handlebody group to the outer automorphism group of the free group with rank g, in terms of length spectra. In general, the preimage of each fully irreducible outer automorphism contains a potentially infinite number of pseudo-Anosov mapping classes. Our study reveals a crucial relationship: for any pseudo-Anosov map in this preimage, its stretch factor must equal or exceed that of the corresponding fully irreducible outer automorphism. Notably, in the case of genus two, we establish that the minimum stretch factor among these pseudo-Anosov maps is less than ten times the stretch factor of the fully irreducible outer automorphism. These results partially address a question by Hensel and have practical implications, including a lower bound for the geodesic counting problem in the genus two handlebody group.

==> header_labeling.tex <==
\makeatletter
\let\c@equation\c@subsection
\makeatother
\numberwithin{equation}{section} 

\makeatletter
\let\c@figure\c@equation
\makeatother
\numberwithin{figure}{section} 


\theoremstyle{plain}
\newtheorem{thm}[equation]{Theorem}
\newtheorem{cor}[equation]{Corollary}
\newtheorem{lem}[equation]{Lemma}
\newtheorem{conj}[equation]{Conjecture}
\newtheorem{prop}[equation]{Proposition}

%%%https://tex.stackexchange.com/questions/291346/marking-the-end-of-a-definition
%%%see egreg's solution.
\theoremstyle{definition}
\newtheorem{defn/}[equation]{Definition}
\newtheorem{ex}[equation]{Example}
\newtheorem{fact}[equation]{Fact}
\newtheorem{ques}[equation]{Question}


%%%https://tex.stackexchange.com/questions/126711/double-slash-close-together
\newcommand{\sslash}{\mathbin{\medslash\mkern-7mu\medslash}}

\newenvironment{defn}
  {\renewcommand\qedsymbol{$\sslash$} 
  \pushQED{\qed} \begin{defn/}}
  {\popQED \end{defn/}}

\theoremstyle{remark}
\newtheorem{rmk/}[equation]{Remark}
\newtheorem*{rmk*}{Remark}
\newtheorem{case}{Case}
\newtheorem*{case*}{Case}
\renewcommand{\thecase}{\Roman{case}}
\newtheorem{claim}[equation]{Claim}
\newtheorem*{claim*}{Claim}


\newenvironment{rmk}
  {\renewcommand{\qedsymbol}{$\sslash$}
   \pushQED{\qed}\begin{rmk/}}
  {\popQED\end{rmk/}}




\newcommand{\refsec}[1]{Section~\ref{Sec:#1}}
\newcommand{\refapp}[1]{Appendix~\ref{App:#1}}
\newcommand{\refthm}[1]{Theorem~\ref{Thm:#1}}
\newcommand{\refcor}[1]{Corollary~\ref{Cor:#1}}
\newcommand{\reflem}[1]{Lemma~\ref{Lem:#1}}
\newcommand{\refprop}[1]{Proposition~\ref{Prop:#1}}
\newcommand{\refclm}[1]{Claim~\ref{Clm:#1}}
\newcommand{\refrmk}[1]{Remark~\ref{Rmk:#1}}
\newcommand{\refexa}[1]{Example~\ref{Exa:#1}}
\newcommand{\reffac}[1]{Fact~\ref{Fac:#1}}
\newcommand{\refque}[1]{Question~\ref{Que:#1}}
\newcommand{\reffig}[1]{Figure~\ref{Fig:#1}}
\newcommand{\reftab}[1]{Table~\ref{Tab:#1}}
\newcommand{\refdefn}[1]{Definition~\ref{Defn:#1}}
\newcommand{\refeqn}[1]{Equation~\ref{Eqn:#1}}
\newcommand{\refconj}[1]{Conjecture~\ref{Conj:#1}}
\newcommand{\refitm}[1]{(\ref{Itm:#1})}



\newcommand{\fakeenv}{} %%% prints the emptystring

%%% For theorem style
\newenvironment{restate}[2]  %%% restate takes two arguments 
{ 
 \renewcommand{\fakeenv}{#2} %%% So now \fakeenv prints #2
 \theoremstyle{plain} 
 \newtheorem*{\fakeenv}{#1~\ref{#2}} %%% so now #2 is the name of a
 %%% theorem-like environment.   
 \begin{\fakeenv}
}
{
 \end{\fakeenv}
}

